Bridging Causal Reversibility and Time Reversibility: A Stochastic Process Algebraic Approach

Causal reversibility blends reversibility and causality for concurrent systems. It indicates that an action can be undone provided that all of its consequences have been undone already, thus making it possible to bring the system back to a past consistent state. Time reversibility is instead considered in the field of stochastic processes, mostly for efficient analysis purposes. A performance model based on a continuous-time Markov chain is time reversible if its stochastic behavior remains the same when the direction of time is reversed. We bridge these two theories of reversibility by showing the conditions under which causal reversibility and time reversibility are both ensured by construction. This is done in the setting of a stochastic process calculus, which is then equipped with a variant of stochastic bisimilarity accounting for both forward and backward directions.

==> Makefile <==
SOURCES = paper.tex intro.tex causal.tex time.tex rmpc.tex bisim.tex examples.tex concl.tex biblio.bib \
	  lmcs.cls macro.sty Commands.tex Makefile

FIGURES = Pictures/causal_time_rev.pdf Pictures/expansion_law.pdf

OBJECTS = *.pdf *.aux *.bbl *.log *.out *.blg Pictures/*.pdf Pictures/*.bak

SUBM_OBJECTS = *.aux *.bbl *.log *.out *.blg Pictures/*.bak

paper.pdf: $(SOURCES) $(FIGURES)
	pdflatex paper.tex
	bibtex paper
	pdflatex paper.tex
	pdflatex paper.tex
	acroread paper.pdf &

Pictures/causal_time_rev.pdf: Pictures/causal_time_rev.fig Makefile
	fig2dev -Lpdf -m0.40 -p1 Pictures/causal_time_rev.fig Pictures/causal_time_rev.pdf

Pictures/expansion_law.pdf: Pictures/expansion_law.fig Makefile
	fig2dev -Lpdf -m0.40 -p1 Pictures/expansion_law.fig Pictures/expansion_law.pdf

clean:
	rm -f $(OBJECTS)

subm_clean:
	rm -f $(SUBM_OBJECTS)

